Representation Learning with Deep Extreme Learning Machines for Efficient Image Set Classification

Efficient and accurate joint representation of a collection of images, that belong to the same class, is a major research challenge for practical image set classification. Existing methods either make prior assumptions about the data structure, or perform heavy computations to learn structure from the data itself. In this paper, we propose an efficient image set representation that does not make any prior assumptions about the structure of the underlying data. We learn the non-linear structure of image sets with Deep Extreme Learning Machines (DELM) that are very efficient and generalize well even on a limited number of training samples. Extensive experiments on a broad range of public datasets for image set classification (Honda/UCSD, CMU Mobo, YouTube Celebrities, Celebrity-1000, ETH-80) show that the proposed algorithm consistently outperforms state-of-the-art image set classification methods both in terms of speed and accuracy.

==> ELM_relatedwork.tex <==
Huang et al. \cite{ELMNC,ELMTNN} proposed the extreme learning machine (ELM) for training SLFNs. 


In contrast to the existing training approaches for SLFNs, ELM only updates the
output weights between the hidden layer and the output layer,
while the input weights and biases of the
hidden layer, are randomly generated. 
The training of the output weights is efficiently performed by solving the regularized least squares.
Using the squared loss of the prediction error, the outputs weights are efficiently trained by solving regularized leas squares. 

ELM  maintains its universal approximation capability \cite{ELMTNN12,ELMTNN06,}


Compared to gradient based algorithms, ELMs are much more efficient and
usually lead to better generalization performance [20]–[22].


==> conclusion.tex <==
\B{still missing}
